Scheduling Battery-Electric Bus Charging under Stochasticity using a Receding-Horizon Approach

A significant challenge of adopting battery electric buses into fleets lies in scheduling the charging, which in turn is complicated by considerations such as timing constraints imposed by routes, long charging times, limited numbers of chargers, and utility cost structures. This work builds on previous network-flow-based charge scheduling approaches and includes both consumption and demand time-of-use costs while accounting for uncontrolled loads on the same meter. Additionally, a variable-rate, non-linear partial charging model compatible with the mixed-integer linear program (MILP) is developed for increased charging fidelity. To respond to feedback in an uncertain environment, the resulting MILP is adapted to a hierarchical receding horizon planner that utilizes a static plan for the day as a reference to follow while reacting to stochasticity on a regular basis. This receding horizon planner is analyzed with Monte-Carlo techniques alongside two other possible planning methods. It is found to provide up to 52\% cost savings compared to a non-time-of-use aware method and significant robustness benefits compared to an optimal open-loop method.

==> architecture.tex <==
\section{Architecture}

This section outlines the architecture of the receding horizon planner, and how it relates to the planning architecture that I have set up.

\begin{figure*}
    \centering
    \includegraphics[width=\linewidth]{images/architecture.jpg}
    \caption{The current planning architecture (the top diagram) and the additions and modifications to it to enable its use in a receding horizon fashion (the bottom diagram), along with the relationship between the two.}
    \label{fig:architecture}
\end{figure*}

In Fig. \ref{fig:architecture} the current planning architecture and the modifications to it for using it as a receding horizon planner are shown. The planning architecture consists of defining a scenario, creating a graph to represent the scenario, converting that graph to a network flow based mixed integer linear program (MILP), solving the MILP, and, finally, extracting the charging plan from the MILP solution. The receding horizon methodology re-utilizes all of these main components, but needs to adjust some aspects of the process (e.g., add a terminal cost, adjust cost based on the previous plan, etc.). 

One of the primary adjustments is that a terminal cost needs to be added to the MILP formulation to help drive the optimal solution back toward a long-term plan (which informs the receding horizon planner about long-term optimal trends for avoiding short-term local optima). Because this terminal cost (and the associated slack variables) does not (in this case at least) invalidate or change the original MILP formulation this adjustment can be done as a separate block that takes the original MILP as input and outputs a new MILP with the terminal cost added in. 

Another adjustment for the receding horizon planner is to reference the plan from the previous horizon and prefer paths that are similar to the previous plan. This helps to reduce oscillations from one horizon to the next between different plans that are very similar in cost. The most natural place to inspect this similarity is in the graph. Each edge in the graph has an associated cost, so by adjusting edges that are similar to the previous plan to have a better cost the resulting MILP will prefer solutions similar to the previous plan. This can be done as a post-process step to the graph creation process, allowing the original graph creation to be un-changed.

The final significant adjustment is creating a warm-start solution to the MILP. This is typically created from the previous plan with a heuristic method for ``filling in'' the portion of the current horizon that is outside the previous horizon's plan. This is what is expected to be the case for this implementation. To allow for other possible methods of constructing a warm-start and to best separate the warm-start details, I plan on having this be like an independent block that receives the graph, the previous plan, and the long-term plan and returns a warm-start solution for the MILP.

The described adjustments are structured the way that they are so that there is little to no adjustment to the methods and blocks that already exist for the non-receding horizon planner. This is so that the original planner can still be used to generate the long-term plans that the receding horizon planner references. Some slight differences between the described adjustments and the block diagram in Fig. \ref{fig:architecture} exist, primarily because the descriptions above treated the adjustments independently, but in reality making the warm-start and adjusting the costs to prefer the previous plan both need to know what edges are ``close'' to the previous plan. Hence, that is separated into it's own block for reuse.

==> graph.tex <==
\subsection{Graph and Network-flow Basics}\label{ssec:graph_basics}
A directed graph \(G\) is defined as a set of vertices, \(V\),  and edges, \(E \subset V \times V\), i.e. \(G =\{V,E\} \).
Given two vertices in the graph, \(v_1, v_2 \in V\), an edge from \(v_1\) to \(v_2\) implies that the ordered pair \((v_1, v_2)\) is in the edge set, i.e., \((v_1, v_2) \in E\).
An example directed graph is shown in \cref{fig:simple_graph}
with four vertices and five edges.

\begin{figure}[!ht]
    \centering
    \includegraphics[width=.4\linewidth]{images/simple_graph_group.jpg}
    \caption{\label{fig:simple_graph}
    Sample {directed graph with groups} where numbered circles show vertices and labeled arrows show directed edges.
    The colored ovals depict groups as discussed in \Cref{ssec:base-constraints}.
    {Edges are colored by the group they enter.}}
    % Red and green edges correspond to the input edges of the groups.}
\end{figure}

A network-flow can be represented by a directed graph.
The vertices of the graph are categorized as \textit{sources}, \textit{sinks}, or \textit{intermediary} vertices.
A source vertex is one that introduces \textit{flow} into the network, while a sink vertex removes it.
The flow then can move from vertex to vertex along edges which are often subject to a capacity constraint.
Each intermediary vertex cannot introduce or remove flow from the network, and so the sum of the flow into the vertex must equal the sum out of the vertex.

As defined in~\cite{Mesbahi2010}, the incidence matrix
%\footnote{The definition of incidence matrix sometimes includes a positive one in both nonzero rows of each column. The incidence matrix as defined in this paper is also referred to as the coefficient matrix \cite{Chen2010}.}
can be used to represent the vertices and edges in matrix form and is denoted as \(D\).
Given \(|V| = n_v\) and \(|E| = n_e\), where \(|\cdot|\) denotes the cardinality of a set, the incidence matrix is of dimension \(n_v \times n_e\).
Each column of \(D\) is used to represent an edge, while each row of \(D\) corresponds to a specific vertex.
Using the notation \(D = [d_{mn}]\) to denote the matrix such that the element in row \(m\) and column \(n\) is \(d_{mn}\), the incidence matrix is defined as
%If edge \(j\) originates at node \(i\) then a \(1\) is placed in \(D\) at row \(i\) column \(j\). If edge \(j\) ends at node \(i\) then a \(-1\) is placed at row \(i\) column \(j\). If edge \(j\) does not include node \(i\) then a \(0\) is placed at row \(i\) column \(j\). This can be written succinctly as
\begin{equation}
    \label{eq:incidence_matrix}
    D = [d_{mn}] \mbox{, } d_{mn} = \begin{cases}
        1  & \mbox{Edge } n \mbox{ begins at vertex } m \\
        -1 & \mbox{Edge } n \mbox{ ends at vertex } m   \\
        0  & \mbox{Otherwise}
    \end{cases}.
\end{equation}
The incidence matrix of the graph in \cref{fig:simple_graph} can be written as
\begin{equation}
    \label{eq:simple_graph_indicidence}
    D = \begin{bmatrix}
        1  & 0  & 0  & 0  & 0  \\
        -1 & 1  & -1 & 0  & 1  \\
        0  & -1 & 1  & 1  & 0  \\
        0  & 0  & 0  & -1 & -1
    \end{bmatrix}.
\end{equation}

Edge indices are taken directly from the incidence matrix using the notation \(e_i\) to represent the edge corresponding to the  \(i^{th}\) column of \(D\).
The edge index set, \(\mathcal{I}\), is the set of integers from \(1\) to \(n_e\).

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Graph-based Representation of Charger Action Space}\label{ssec:charger_graph}
For the purposes of this work, the routes of the BEBs are assumed to be fixed and known a priori.
This allows abstracting each BEB's route schedule to focus primarily on the times when it will be available to charge.
Additionally, it permits grouping any chargers that are in the same location and that have the same characteristics together into a \textit{charger type}.
To illustrate these simplifications, take as example a bus that starts its day leaving from the depot at 5 AM and begins a route.
It then stops at a station (Station A) that has only fast chargers at 6 AM for 10 minutes before continuing on its next route.
Then, it stops at another station (Station B) that has both slow and fast chargers at 7 AM for 15 minutes.
Afterward, the bus departs to run the first route again and continues the cycle until 9 PM when it returns to the depot for the night.
In this example, the fast chargers at Station A are grouped as charger type 1, the slow chargers at Station B are grouped as charger type 2 and the fast chargers at Station B are grouped as charger type 3.
The main component of the BEB's charging schedule is specifying that it is available to charge at charger type 1 from 6 to 6:10 AM and at charger types 2 and 3 from 7 to 7:15 AM, and so on through the day.

In this work, the flow of the network represents the ``flow'' of chargers from one charging task to another.
Each vertex corresponds to a particular charger type either charging a particular bus at a particular point in time or doing nothing at that time.
As each vertex is associated with an instant in time, the charger actions, e.g., charging or not, occur along the edges.
There are three types of actions that edges can represent:
\begin{itemize}
    \item Edges between two charging vertices of a bus correspond to the bus being charged by a charger of the corresponding type
    \item Edges between two rest vertices correspond to a charger doing nothing
    \item Edges between charging and rest vertices represent a charger transitioning to/from rest from/to charging a given bus
\end{itemize}
A vertex is only present in the graph when a bus will be available to charge with the corresponding charger type.

A simplified example of such a graph is shown in \cref{fig:bus_nodes} and follows the schedule of the bus in the previous example, with additional buses for illustration purposes.
The sub-graph in \cref{fig:bus_nodes} consists only of the vertices corresponding to charger type 1, the full graph consists of a similar sub-graph for each charger type.
There are vertices for the bus of the example at 6, 6:05, and 6:10 AM representing that the bus is available to charge with charger type 1 during those times.
These are grouped together (represented with an orange oval) as one \textit{visit} to the station.
The vertices of a later visit to the station would be grouped together separately from this group (as Bus 2 shows in \cref{fig:bus_nodes}).
Vertices that correspond to a different charger type at the same station, however, would be grouped together as part of the same visit.

\begin{figure}[!
        ht]
    \centering
    \includegraphics[width=.9\linewidth]{images/ExampleBusChargeGraph.pdf}
    \caption{\label{fig:bus_nodes}
        A graph depicting the possible state and transitions for a single charger type over time for a simple {bus charging} example.
        The bottom row corresponds to the charger at rest while the other rows each correspond to charging a particular bus.
        Yellow ovals {show the vertex groups that} are placed around charging windows.
    }
\end{figure}

All chargers of the same type and at the same station can be represented by a single connected sub-graph in the network flow formulation.
Edges corresponding to a charger resting are allowed to have an edge flow up to the number of chargers, while edges ending at charging vertices are restricted to allow up to a unit flow.
A separate sub-graph is used for each charger type to allow the edges to correspond to different charging rates, costs, locations, etc. Constraints are added to enforce that only one charger can charge a bus at any given time.


==> litreview.tex <==
\section{Literature Review}\label{sec:lit-review}
The problem of scheduling the charging of BEBs has received significant attention in the literature.
A great body of the literature is based on adapting the vehicle routing/scheduling problem (VRP/VSP) to represent and solve the problem.
%with the work in~\cite{Li2014} being a seminal adaptation of the VSP for the BEB charge scheduling problem.
In~\cite{Li2014}, a seminal work in the field, a single-depot VSP (SD-VSP) for scheduling BEB charging is formulated with a network flow-based model,
% Each node represents either charging for some time period or going on a route; edges signify transitions between these activities.
and solved with a custom branch-and-price framework.
A large portion of the BEB literature can be viewed as extensions to~\cite{Li2014} that address additional considerations.
The extensions to~\cite{Li2014} that are most relevant to the proposed method can be categorized into: \textit{utility costs},
%\textit{mixed-fleet},
\textit{partial charging}, and \textit{stochastic awareness}.
An overview of representative works with relation to these categories is shown in~\Cref{tab:literature}.

% Please add the following required packages to your document preamble:
% \usepackage{booktabs}


The most common extensions of the problem are related to improved models of utility costs.
For example,~\cite{Zhou2020-Mixed,Rinaldi2020,He2020,Bagherinezhad2020} adapt~\cite{Li2014} to directly account for the battery capacity instead of the remaining range and extend the cost to include time-of-use (TOU) and demand rates.
Many works have included consumption in their cost functions~\cite{Rinaldi2020,Zhou2020-Mixed,Zhang2021,Duan2021,Bie2021,Tang2019}, with some explicitly considering TOU rate schedules~\cite{Zhou2020-Mixed,Rinaldi2020}.
A few have also considered demand costs~\cite{He2020,Bagherinezhad2020,Mortensen2023}.
While often not considered, demand costs typically account for a significant percentage of the overall charging costs when they are included in the utility's rate schedule~\cite{Qin2016}.

% Considering mixed fleets of electric buses and internal combustion buses is the focus of~\cite{Zhou2020-Mixed, Rinaldi2020, Duan2021, Zhou2020}.
% These works include scheduling both traditional diesel buses and BEBs to routes, while only the BEBs are scheduled to charge.

% Extensions to~\cite{Li2014} that are particularly significant to this work account for the stochasticity of real-world operations, e.g.,~\cite{Duan2021,Bie2021,Tang2019}.
% The works~\cite{Duan2021,Bie2021} extend~\cite{Li2014} to account for stochastic arrival times in a static, or open-loop, fashion (no feedback).
% In contrast,~\cite{Tang2019} extends~\cite{Li2014} with a dynamic, receding horizon approach that receives feedback to account for delayed BEB arrival times and charge level discrepancies.

A major assumption~\cite{Li2014} and many others have is that a vehicle always charges to full charge within the scheduled time irrespective of the state of charge level or the duration of the charge event.
In contrast, modeling partial charging can help BEBs share limited chargers more effectively, can result in much reduced demand costs, and can allow higher fidelity charging models.
% A more accurate non-linear charging profile can reduce costs and ensure low charge level constraints are enforced.
Considering partial charging enabled~\cite{He2020,Bagherinezhad2020,Mortensen2023} to provide models of the energy and power usages to calculate TOU consumption and demand costs, improving costs significantly.
Even in the few works that allow partial charging, it is most common to use a linear charge profile~\cite{Chen2016,Bagherinezhad2020,Mortensen2023}.
In~\cite{Zhang2021}, the authors model partial charging with the specific purpose of modeling non-linear charging profiles and battery health considerations.
However, the computational burden of~\cite{Zhang2021} is high.
A non-linear charging profile method is used in~\cite{Whitaker23} that is not as computationally burdensome, but that is only an approximation of a typical constant-current/constant-voltage charging profile.
% This also allowed~\cite{He2020,Bagherinezhad2020,Mortensen2023} to model both TOU consumption and TOU demand costs.

% While~\cite{Li2014}, extensions to it, and similar works primarily focus on scheduling both charging and BEB-to-route assignments, there are some works that simplify the problem with fixed, a priori BEB-to-route assignments.
% Several works approach solving this simplified problem in a heuristic manner.
% In~\cite{Qin2016}, a thresholding and queuing method is presented that allows for simple decisions to govern charging.
% The algorithm of~\cite{Frendo2021} distributes available power as evenly among connected BEBs as possible within the limits of the system, and recomputes solutions as BEBs enter and leave.
% Two bin-packing inspired heuristic algorithms are proposed in~\cite{Jahic2019} that determine charging start and stop times for BEBs at three power levels.
% In contrast, the works of~\cite{ Chen2016, Bagherinezhad2020, He2020, Mortensen2023} form optimal solutions to variations of the fixed-schedule problem, with~\cite{Chen2016} additionally considering other loads on the distribution system.

Most of the works in the literature consider the problem without any stochastic awareness, where all necessary information is known a priori and the resulting solution can be executed exactly.
There are, however, a number of works that account for the inherent stochastic nature of the problem.
Several works take the approach of solving \textit{static} problems, with only \textit{a priori} information, that attempt to be robust to the possible sources of noise~\cite{Tang2019,Bie2021,Duan2021}.
\cite{Tang2019} adds a buffer time to the scheduled end of each route to ensure robustness to traffic delays. % chktex 2
The approach in~\cite{Bie2021} considers stochastic energy consumption along routes as well as possible traffic delays and formulates an optimization problem that minimizes the expected energy consumption and expected departure delays while providing a robust charging plan.
Similarly,~\cite{Duan2021} forms a robust optimization problem that considers energy consumption and traffic delays, but extends it to a mixed fleet of conventional buses and BEBs.
In contrast, others solve the problem in a \textit{dynamic} way by periodically re-solving the problem; this allows the solution to adapt to feedback~\cite{Tang2019,Wang2019,Wang2021}.
\cite{Tang2019} repeatedly solves the problem considering operation and delay costs over a short horizon, applying only the first portion of each solution before receiving feedback and re-solving in a receding-horizon manner. % chktex 2
The authors of~\cite{Wang2019,Wang2021} use an optimal policy derived from a Markov decision process (MDP) that models the choices each vehicle can make when in the station.
At each point in time, a policy iteration algorithm rapidly finds the optimal choice for a vehicle to make given the most up-to-date feedback and data available.

However, methods that address stochasticity lag behind the state-of-the-art methods that do not consider stochasticity.
While non-stochastic approaches have addressed TOU demand costs in addition to TOU consumption costs, the stochastic approaches, as far as we have found, have not yet included TOU demand costs.
Additionally, no stochastically aware methods were found that use partial charging models.
Furthermore,~\cite{Wang2019,Wang2021} require large quantities of data to accurately model the costs and probabilities in the MDP\@.
This restricts the method's usefulness in cases where the requisite data is not available (for example, when first integrating BEBs into operations) or whenever there are significant changes that invalidate data (for example, if schedules, BEB models/characteristics, typical traffic conditions, etc.\ change).

The literature for BEB charge scheduling that considers stochasticity, therefore, lacks a method that considers both TOU consumption and TOU demand costs with a non-linear partial charging model in a method that can readily adapt to changes in the underlying scenario (e.g., schedules, BEB models).
The contained work seeks to fill this gap by considering full TOU utility costs with a non-linear, variable-rate partial charging model in a dynamic receding horizon methodology that can not only react to stochasticity but also be adapted to match systemic changes.

% A large portion of the fixed- and flexible-schedule methods solve the problem using classical optimization techniques.
% This is a good approach for small- and sometimes medium-sized problems, but does not scale to large problem sizes due to the integer constraints on some variables of optimization in nearly all formulations of the problem~\cite{Sassi2016}.
% The work in~\cite{He2020} is a notable exception as its method results in a fully continuous linear program which can be solved rapidly.
% The authors of~\cite{He2020}, however, leveraged the assumption that there was no scarcity of chargers (i.e., a bus may charge whenever necessary) in order to achieve this.
% Otherwise, there have been a number of other approaches that have been taken to allow for rapid solutions to the problem, generally split between meta-heuristic~\cite{Alonso2014,Wen2016,Varga2022} and heuristic approaches~\cite{Qin2016,Jahic2019,Sassi2016,Tucker2019,Frendo2021}.
% For the meta-heuristic methods,~\cite{Alonso2014} uses a genetic algorithm to solve the problem, while~\cite{Wen2016,Varga2022} both perform neighborhood searches based on the MILP formulation of the problem.
% The heuristic methods include~\cite{Qin2016}, which uses a thresholding technique that determines if a bus should charge depending on whether its state of charge is above a certain threshold or not.
% Additionally,~\cite{Qin2016} determines an optimal threshold value for the specific scenario studied.
% Three heuristic approaches were proposed in~\cite{Jahic2019} that attempt to schedule charging in fixed or variable duration blocks for each bus.
% The three heuristics differ in the amount of variability in the block width and whether the blocks can be scheduled in one or two chunks.
% Two heuristics derived from optimization formulations are given in~\cite{Sassi2016}; the first considering vehicles sequentially, while the second solves the assignment of routes to vehicles first, then solves for the optimal charging schedule.

